Adversarially Regularized Graph Autoencoder for Graph Embedding

Graph embedding is an effective method to represent graph data in a low dimensional space for graph analytics. Most existing embedding algorithms typically focus on preserving the topological structure or minimizing the reconstruction errors of graph data, but they have mostly ignored the data distribution of the latent codes from the graphs, which often results in inferior embedding in real-world graph data. In this paper, we propose a novel adversarial graph embedding framework for graph data. The framework encodes the topological structure and node content in a graph to a compact representation, on which a decoder is trained to reconstruct the graph structure. Furthermore, the latent representation is enforced to match a prior distribution via an adversarial training scheme. To learn a robust embedding, two variants of adversarial approaches, adversarially regularized graph autoencoder (ARGA) and adversarially regularized variational graph autoencoder (ARVGA), are developed. Experimental studies on real-world graphs validate our design and demonstrate that our algorithms outperform baselines by a wide margin in link prediction, graph clustering, and graph visualization tasks.

==> noise_link_pred.tex <==
\begin{table*}[htpb]
\small
  \centering
  \caption{Experimental Results on Noised Link Prediction}
%   \begin{tabular}{c{2cm}c{1.7cm}c{1.7cm}c{1.7cm}c{1.7cm}c{1.7cm}c{1.7cm}}
\begin{tabular}{ccccccc}
\hline
 Approaches & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{Citeseer}& \multicolumn{2}{c}{Pubmed} \\
& AUC & AP& AUC & AP& AUC & AP\\
SC &	00.0 $\pm$  0.01 &	00.0 $\pm$ 0.00 &	00.0 $\pm$  0.01 &	00.0 $\pm$  0.01 &	00.0 $\pm$  0.02 &	00.0 $\pm$  0.01\\
DW &	00.0 $\pm$  0.01 &	00.0 $\pm$  0.00 &	00.0 $\pm$ 0.02 &	00.0 $\pm$  0.01 &	00.0 $\pm$  0.00 &	00.0 $\pm$  0.00\\
      \midrule
$GAE^*$ &	86.9 $\pm$  0.02 &	89.6 $\pm$  0.01 &	75.7 $\pm$  0.02 &	82.0 $\pm$  0.02 &	82.8 $\pm$  0.01 &	87.9 $\pm$  0.00\\
$VGAE^*$ &	85.7 $\pm$  0.02 &	89.0 $\pm$  0.01 &	78.3 $\pm$  0.03 &	84.1 $\pm$  0.02 &	82.4 $\pm$  0.01 &	87.4 $\pm$  0.01\\
GAE &	91.3 $\pm$  0.02 &	92.8 $\pm$  0.03 &	88.3 $\pm$  0.04 &	89.3 $\pm$  0.05 &	95.4 $\pm$  0.00 &	95.7 $\pm$  0.00\\
VGAE &	91.0 $\pm$  0.01 &	92.6 $\pm$  0.01 &	89.8 $\pm$  0.02 &	91.5 $\pm$  0.02 &	93.9 $\pm$  0.02 &	94.2 $\pm$  0.02\\
        \midrule
\textbf{ARGE} &	92.4 $\pm$  0.003 &	\textbf{93.2 $\pm$  0.003} &	91.9 $\pm$  0.003 &	93.0$\pm$  0.003 &	\textbf{96.9 $\pm$  0.001} &	\textbf{97.2 $\pm$  0.001}\\
\textbf{ARVGE} &	\textbf{91.6 $\pm$  0.004} &	93.0 $\pm$  0.004 &	\textbf{91.0 $\pm$  0.003} &	\textbf{92.0 $\pm$  0.003} &	95.7$\pm$  0.001 &	96.0$\pm$  0.001\\
\hline
\end{tabular}

  \label{tab:noisedlinkprediction}%
\end{table*}%
